SFT Memorizes, RL Generalizes: A Comparative Study of Foundation Model Post-training

Supervised fine-tuning (SFT) and reinforcement learning (RL) are widely used post-training techniques for foundation models. However, their roles in enhancing model generalization capabilities remain unclear. This paper studies the difference between SFT and RL on generalization and memorization, focusing on text-based rule variants and visual variants. We introduce GeneralPoints, an arithmetic reasoning card game, and adopt V-IRL, a real-world navigation environment, to assess how models trained with SFT and RL generalize to unseen variants in both textual and visual domains. We show that RL, especially when trained with an outcome-based reward, generalizes across both rule-based textual and visual variants. SFT, in contrast, tends to memorize training data and struggles to generalize out-of-distribution scenarios. Further analysis reveals that RL improves the model's underlying visual recognition capabilities, contributing to its enhanced generalization in the visual domain. Despite RL's superior generalization, we show that SFT remains essential for effective RL training; SFT stabilizes the model's output format, enabling subsequent RL to achieve its performance gains. These findings demonstrates the capability of RL for acquiring generalizable knowledge in complex, multi-modal tasks.

==> Tex/method.tex <==
\begin{center}
    \centering
    \captionsetup{type=figure}    
    \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]  % No padding around the node
      \node (image) {\includegraphics[width=.7\textwidth]{figures/method-pipeline.pdf}};
      \node[draw, fit=(image), inner sep=2pt] {}; % Draw a frame with 5pt inner padding
    \end{tikzpicture}
  \caption{\small {\bf An example of our overall method pipeline.}}
  \label{fig:method-pipeline}
\end{center}


\sz{writing here, next need to discuss about the entire pipeline. Things to consider

\begin{itemize}
    \item Parallel best of N versus our stacked history of N trajs
    \item 
\end{itemize}
}



\begin{algorithm}[ht]
\caption{Improving Reasoning Pipeline (temp)}\label{algo:name-tbd} \sz{this is just a template, need to update it later}
\begin{algorithmic}[1]

\State \textbf{Input:} An environment $\tt{env}$, an initial VLM with parameters $\theta_{0}$.
\State \textbf{Input:} A post-processing function $f$, a CoT reasoning scaling factor $\lambda$.
\State \textbf{Input:} Replay buffer size $B$, maximum episode length $T$.  
\For{$k=0,\dots,K-1$} 
    
    \State $t=0$ \Comment{Reset RL time step}
    \State $o_t = \tt{env.reset()}$ \Comment{Reset the initial state}
    \State $\vin_t = h(o_t)$ 
    \State $\mc B_k = \emptyset$ \Comment{Initialize an on-policy replay buffer}
    \While{$|\mc B_k|\leq B$}
    \State $\vout_t = \pi_{\theta_k}(o_t,\vin_t)$ \Comment{Generate text output}
    \State $a_t = f(\vout_t)$ 
    \State $\log \pi_{\theta_k}(a_t|o_t,\vin_t) = \lambda\log \pi_{\theta_k}(\blue{\vtht_t}|\vin_t) + \log \pi_{\theta_k}(\red{\vact_t}|o_t,\vin_t,\vtht_t)$ 
    \State $r_t,o_{t+1} = {\tt env.step}(a_t)$
    \State $\mc B_k = \mc B_k\cup\{(o_t,a_t,r_t,\vout_t,\log\pi_{\theta_k}(a_t|o_t,\vin_t))\}$ \Comment{Add data to the buffer $\mc B_k$}
    \State $t=t+1$
    \If{$t=T$}
        \State $t=0$ 
    \Comment{Reset RL time step if the maximum step is reached}
        \State $o_0 = {\tt env.reset()}$ \Comment{Reset environment}
    \EndIf
    \State $\vin_t = h(o_t)$ \Comment{Prepare the next $\vin_t$}    
    \EndWhile
    \State Run PPO~\citep{schulman2017proximal} with data $\mc B_k$ to obtain $\theta_{k+1}$
\EndFor
\State \textbf{Output:} $\theta_K$.
\end{algorithmic}
\end{algorithm}

